Minimally subtracted six loop renormalization of $O(n)$-symmetric $\phi^4$ theory and critical exponents

We present the perturbative renormalization group functions of $O(n)$-symmetric $\phi^4$ theory in $4-2\varepsilon$ dimensions to the sixth loop order in the minimal subtraction scheme. In addition, we estimate diagrams without subdivergences up to 11 loops and compare these results with the asymptotic behaviour of the beta function. Furthermore, we perform a resummation to obtain estimates for critical exponents in three and two dimensions.

==> beta.tex <==
- 2 \eps g
+\frac{\n+8}{3}g^2
-\frac{3 \n +14}{3}g^3
+\frac{
    96 (5 \n+22) \mzv{3}
  + 33 \n^2 +922 \n + \numprint{2960}
}{216}g^4 % \frac{g^4}{216}
\\&
-\Big[
	\numprint{1920} (
		2 \n^2
		+55 \n
		+186 
	) \mzv{5}
	-288 (
		\n
		+8 
	) (
		5 \n
		+22 
	) \mzv{4}
\\&\quad
	+96 (
		63 \n^2
		+764 \n
		+\numprint{2332} 
	) \mzv{3}
	- (
		5 \n^3
		-\numprint{6320} \n^2
		-\numprint{80456} \n
		-\numprint{196648} 
	) 
\Big] \frac{g^5}{\numprint{3888}}
\\&
+\Big[
	\numprint{112896} (
		14 \n^2
		+189 \n
		+526 
	) \mzv{7}
	-768 (
		6 \n^3
		+59 \n^2
		-446 \n
		-\numprint{3264} 
	) \mzv[2]{3}
\\&\quad
	-\numprint{9600} (
		\n
		+8 
	) (
		2 \n^2
		+55 \n
		+186 
	) \mzv{6}
	+256 (
		305 \n^3
		+\numprint{7466} \n^2
		+\numprint{66986} \n
		+\numprint{165084} 
	) \mzv{5}
\\&\quad
	-288 (
		63 \n^3
		+\numprint{1388} \n^2
		+\numprint{9532} \n
		+\numprint{21120} 
	) \mzv{4}
\\&\quad
	-16 (
		9 \n^4
		-\numprint{1248} \n^3
		-\numprint{67640} \n^2
		-\numprint{552280} \n
		-\numprint{1314336} 
	) \mzv{3}
\\&\quad
	+ (
		13 \n^4
		+\numprint{12578} \n^3
		+\numprint{808496} \n^2
		+\numprint{6646336} \n
		+\numprint{13177344} 
	) 
\Big] \frac{g^6}{\numprint{62208}}
\\&
-\Big[
	\numprint{204800} (
		\numprint{1819} \n^3
		+\numprint{97823} \n^2
		+\numprint{901051} \n
		+\numprint{2150774} 
	) \mzv{9}
\\&\quad
	+\numprint{14745600} (
		\n^3
		+65 \n^2
		+619 \n
		+\numprint{1502} 
	) \mzv[3]{3}
\\&\quad
	+\numprint{995328} (
		42 \n^3
		+\numprint{2623} \n^2
		+\numprint{25074} \n
		+\numprint{59984} 
	) \mzv{3,5}
\\&\quad
	-\numprint{20736} (
		\numprint{28882} \n^3
		+\numprint{820483} \n^2
		+\numprint{6403754} \n
		+\numprint{14174864} 
	) \mzv{8}
\\&\quad
	-\numprint{5529600} (
		8 \n^3
		-635 \n^2
		-\numprint{9150} \n
		-\numprint{25944} 
	) \mzv{3}\mzv{5}
\\&\quad
	+\numprint{11520} (
		440 \n^4
		+\numprint{126695} \n^3
		+\numprint{2181660} \n^2
		+\numprint{14313152} \n
		+\numprint{29762136} 
	) \mzv{7}
\\&\quad
	+\numprint{207360} (
		\n
		+8 
	) (
		6 \n^3
		+59 \n^2
		-446 \n
		-\numprint{3264} 
	) \mzv{3}\mzv{4}
\\&\quad
	-\numprint{23040} (
		188 \n^4
		+132 \n^3
		-\numprint{93363} \n^2
		-\numprint{862604} \n
		-\numprint{2207484} 
	) \mzv[2]{3}
\\&\quad
	-\numprint{28800} (
		595 \n^4
		+\numprint{20286} \n^3
		+\numprint{277914} \n^2
		+\numprint{1580792} \n
		+\numprint{2998152} 
	) \mzv{6}
\\&\quad
	+\numprint{5760} (
		\numprint{4698} \n^4
		+\numprint{131827} \n^3
		+\numprint{2250906} \n^2
		+\numprint{14657556} \n
		+\numprint{29409080} 
	) \mzv{5}
\\&\quad
	+\numprint{2160} (
		9 \n^5
		-\numprint{1176} \n^4
		-\numprint{88964} \n^3
		-\numprint{1283840} \n^2
		-\numprint{6794096} \n
		-\numprint{12473568} 
	) \mzv{4}
\\&\quad
	-720 (
		33 \n^5
		+\numprint{2970} \n^4
		-\numprint{477740} \n^3
		-\numprint{10084168} \n^2
		-\numprint{61017200} \n
		-\numprint{117867424} 
	) \mzv{3}
\\&\quad
	-45 (
		29 \n^5
		+\numprint{22644} \n^4
		-\numprint{3225892} \n^3
		-\numprint{88418816} \n^2
		-\numprint{536820560} \n
		-\numprint{897712992} 
	) 
\Big] \frac{g^7}{\numprint{41990400}}
\\&
+\bigo{g^8}


==> gammaM2.tex <==
-\frac{(n+2)g}{3}
+\frac{5(n+2) g^{2}}{18}
- \frac{(5n+37)(n+2)g^3}{36}
\\&
+\Big[
	\numprint{288}
	(
		5\n
		+22
	) \mzv{4}
	+\numprint{48}
	(
		3\n^{2}
		+10\n
		+68
	) \mzv{3}
%\\&\quad
	-
	(
		\n^{2}
		-\numprint{7578}\n
		-\numprint{31060}
	) 
\Big] \frac{(n+2) g^{4}}{\numprint{7776}}
\\&
-\Big[
	\numprint{9600}
	(
		2\n^{2}
		+55\n
		+186
	) \mzv{6}
	-\numprint{768}
	(
		2\n^{2}
		+145\n
		+582
	) \mzv[2]{3}
%\\&\quad
	-\numprint{768}
	(
		5\n^{2}
		-14\n
		-72
	) \mzv{5}
\\&\quad
	-\numprint{288}
	(
		3\n^{3}
		-29\n^{2}
		-816\n
		-\numprint{2668}
	) \mzv{4}
%\\&\quad
	+\numprint{48}
	(
		17\n^{3}
		+940\n^{2}
		+\numprint{8208}\n
		+\numprint{31848}
	) \mzv{3}
\\&\quad
	+
	(
		21\n^{3}
		+\numprint{45254}\n^{2}
		+\numprint{1077120}\n
		+\numprint{3166528}
	) 
\Big] \frac{(n+2) g^{5}}{\numprint{186624}}
\\&
+\Big[
	\numprint{1152}
	(
		14\n^{2}
		+189\n
		+526
	)
	(
		2063\mzv{8}
		-144\mzv{3,5}
	)
	-\numprint{921600}
	(
		15\n^{2}
		+239\n
		+718
	) \mzv{3}\mzv{5}
\\&\quad
	-\numprint{640}
	(
		\numprint{1080}\n^{3}
		+\numprint{25180}\n^{2}
		+\numprint{284525}\n
		+\numprint{814062}
	) \mzv{7}
\\&\quad
	-\numprint{15360}
	(
		2\n^{3}
		-157\n^{2}
		-\numprint{2512}\n
		-\numprint{8268}
	) \mzv{3}\mzv{4}
\\&\quad
	+\numprint{5120}
	(
		27\n^{3}
		+\numprint{1082}\n^{2}
		+\numprint{13072}\n
		+\numprint{40008}
	) \mzv[2]{3}
\\&\quad
	+\numprint{3200}
	(
		285\n^{3}
		+\numprint{7178}\n^{2}
		+\numprint{73768}\n
		+\numprint{196032}
	) \mzv{6}
\\&\quad
	+\numprint{320}
	(
		45\n^{4}
		+\numprint{3622}\n^{3}
		+\numprint{12202}\n^{2}
		+\numprint{207708}\n
		+\numprint{753040}
	) \mzv{5}
\\&\quad
	-\numprint{240}
	(
		47\n^{4}
		+\numprint{2606}\n^{3}
		-\numprint{5480}\n^{2}
		-\numprint{194320}\n
		-\numprint{489328}
	) \mzv{4}
\\&\quad
	-\numprint{80}
	(
		51\n^{4}
		-\numprint{9208}\n^{3}
		-\numprint{419076}\n^{2}
		-\numprint{3342688}\n
		-\numprint{8997136}
	) \mzv{3}
\\&\quad
	-\numprint{5}
	(
		43\n^{4}
		+\numprint{48234}\n^{3}
		-\numprint{5154216}\n^{2}
		-\numprint{63140784}\n
		-\numprint{145482928}
	) 
\Big] \frac{(n+2) g^{6}}{\numprint{9331200}}
\\&
+\bigo{g^{7}}


==> gammaPhi.tex <==
\frac{n+2}{36} g^2
-\frac{(n+8)(n+2)}{432} g^3
-\frac{5(n^2-18n-100)(n+2)}{\numprint{5184}}g^4
\\&
-\Big[
	\numprint{1152}
	(
		5\n
		+22
	) \mzv{4}
	-\numprint{48}
	(
		\n^{3}
		-6\n^{2}
		+64\n
		+184
	) \mzv{3}
\\&\quad
	+
	(
		39\n^{3}
		+296\n^{2}
		+\numprint{22752}\n
		+\numprint{77056}
	) 
\Big] \frac{(n+2) g^{5}}{\numprint{186624}}
\\&
-\Big[
	\numprint{512}
	(
		2\n^{2}
		+55\n
		+186
	) \mzv[2]{3}
	-\numprint{6400}
	(
		2\n^{2}
		+55\n
		+186
	) \mzv{6}
\\&\quad
	+\numprint{4736}
	(
		\n
		+8
	)
	(
		5\n
		+22
	) \mzv{5}
%\\&\quad
	-\numprint{48}
	(
		\n^{4}
		+2\n^{3}
		+328\n^{2}
		+\numprint{4496}\n
		+\numprint{12912}
	) \mzv{4}
\\&\quad
	+\numprint{16}
	(
		\n^{4}
		-936\n^{2}
		-\numprint{4368}\n
		-\numprint{18592}
	) \mzv{3}
\\&\quad
	+
	(
		29\n^{4}
		+794\n^{3}
		-\numprint{30184}\n^{2}
		-\numprint{549104}\n
		-\numprint{1410544}
	) 
\Big] \frac{(n+2)g^{6}}{\numprint{746496}}
%\\&
+\bigo{g^{7}}

